Assessment of Source Code Obfuscation Techniques

Obfuscation techniques are a general category of software protections widely adopted to prevent malicious tampering of the code by making applications more difficult to understand and thus harder to modify. Obfuscation techniques are divided in code and data obfuscation, depending on the protected asset. While preliminary empirical studies have been conducted to determine the impact of code obfuscation, our work aims at assessing the effectiveness and efficiency in preventing attacks of a specific data obfuscation technique - VarMerge. We conducted an experiment with student participants performing two attack tasks on clear and obfuscated versions of two applications written in C. The experiment showed a significant effect of data obfuscation on both the time required to complete and the successful attack efficiency. An application with VarMerge reduces by six times the number of successful attacks per unit of time. This outcome provides a practical clue that can be used when applying software protections based on data obfuscation.

==> 05-ss-lessons-learned.tex <==
The experiment preparation has been a crucial phase of the overall experiment.
We took care at this step in order to minimise the possible issues that could arise
during the practical execution of the experiment.

In order to reduce the probability of practical problems we tested the experiment objects
in two different laboratories, out of 9 general purpose computer labs available in the main campus.
Unfortunately, the actual laboratory was known only shortly before the experiment
day and it turned out to be different from both the two tested laboratories.
This fact led to the first practical issue: the operating system of the experiment
laboratory was different from the testing laboratories.
The testing laboratories used a 64-bits Operating System (OS) while the actual lab used a 32-bit OS; the compiler working in the former provided a \texttt{long} variables with size equal to 8 bytes and \texttt{int} variables with size equal to 4 bytes, while in the latter lab
both \texttt{long} and \texttt{int} variables were 4 bytes long
(this is compatible with the ANSI C99 standard~\cite{C99} that specifies only the minimum size of the variable types: 4 bytes for  \texttt{long} variables).
The main consequence of this misalignment appeared when variables were manipulated by the obfuscator:
as described in Section~\ref{sec:obfuscation}, the  \var obfuscation takes two shorter (e.g.,  \texttt{int})
variables and merges them into a unique, longer (e.g., \texttt{long}) variable. Indeed, the implementation of \var that was used makes the assumption that \texttt{long} variables are allocated a memory space that is twice that of \texttt{int}.
% It must be taken into account that the actual OS could not be foreseen in advance because the laboratory machines load a fresh and clean image from the network at startup time.

As a result, the tested obfuscated tasks did not work in the final laboratory.
We addressed the problem directly during the experiment by adapting the assigned source code and converting
the \texttt{long} variables to \texttt{long long} ones.
This hitch caused a minor loss of time (less than five minutes) for those subjects that first reported the anomaly.
We compensated for this issue by asking them to subtract the time lost during the fixing from the overall
task duration.

For future experiments it may be worth to adopt countermeasures to prevent this kind of problems such as:
\begin{itemize}
	\item ensure the target OS is the expected one;
	\item use system independent data types for developing the object applications and their protections (e.g. \texttt{stdint.h}
	types for C language under UNIX systems);
	\item use portable solutions, such as virtual machines or container based systems.
\end{itemize}

\textcolor{red}{The use of post-questionnaires limited our possibility to an objective and precise estimation of the activities that subjects performed. 
This limitation affected our possibility to infer the reasons for unsuccessful attacks, the exact amount of time spent with the different categories of tools, and the attack strategy subjects used to successfully mount an attack.
%
This is another hints to decide to use virtual machines for the next experiments. 
In this way, the experiment's  environment can be equipped with software able to acquire periodic snapshots of the activities conducted, like information on process status and screen-shots that may reveal which are the actually used tools.
}

Apart from the technical issue, the main degree of uncertainty is related to human factors.
First of all, psychological conditioning of the subjects can influence the goodness of the collected data.
The Lotto clear task ($\task[1]$)  was very simple. Indeed, it just required to find
the content of an array by reading the given source code.
Such a trivial task was unexpected and triggered in some subjects doubts about the correctness of their
easy-spotted solution. When such doubts emerged we promptly reassured the participants that they actually found the right solution and so they could proceed.


%Such subjects might have spent some extra time in the unnecessary attempt to figure out  alternative attacks or to double check the overly easy solution that they found.
%In fact, this consideration pushed them to look for other ways of resolution for the remaining 80 minutes of the
%given time even if they found the right solution within the first 10 minutes.
%\todo[inline]{Scritto cos\`i sembra che tutti abbiano girato a vuoto per 80 minuti..., mi pare si sia trattato di 1 o 2 casi.}
%Some of them might have believed that the task was not correctly completed, because they evaluated the assignment to be too easy  compared to the available time.
%\todo[inline]{C'era qualche altro caso legato al fattore umano che mi sfugge??}

%The issues above introduced, directly or indirectly, some noise that possibly increased the task completion time. However, the artificially increased times affected only the clear code. Hence, we expect even stronger results if such unnecessary time increase could be ruled out.

%%
%% Questo rischia di essere frainteso, meglio non riportarlo
%%
%For what concerns the time allotted
%to subjects for carrying out the tasks,
%we originally planned to allocate half session  for the first sub-session (first task) and the
%other half for the second one.
%The forecast was not met, as we observed that as the first sub-session end was getting closer,
%more than  half of the subjects had not yet delivered any solution.
%So, we decided to extend the first half of the experiment while reducing the second part.
%The delay in first sub-session completion was due to a time loss in the very beginning for setting up the
%environment and getting into the problem.
%It is worth to keep in mind that subjects were neither advised about the topic of the task nor
%trained to perform such tasks. Hence, they had to spend some initial time to focus on the task topics.
%The reported data analysis shows that the unbalanced sub-session duration times did not influence the
%correctness or the completion time of tasks.
%
%For future similar experiments, it is advisable to foresee a short early time slot to let
%all the contingent environment factors to converge to a stable initial state from which the
%experimental could begin.

%In conclusion, from this  experience we learned two main lessons:
%
%\begin{itemize}
%	
%	\item during the preparation phase it is necessary to be prepared for the practical
%	issues that can arise during the experiment, being aware that anyway unanticipted issues may always happen;
%	
%	\item assigned time must be evaluated carefully, considering the time for actual performing the
%	tasks, the setup time and further additional time for accidents and issue solving.	
%\end{itemize}
%



